A Dynamic Game Approach for Demand-Side Management: Scheduling Energy Storage with Forecasting Errors

Smart metering infrastructure allows for two-way communication and power transfer. Based on this promising technology, we propose a demand-side management (DSM) scheme for a residential neighbourhood of prosumers. Its core is a discrete time dynamic game to schedule individually owned home energy storage. The system model includes an advanced battery model, local generation of renewable energy, and forecasting errors for demand and generation. We derive a closed-form solution for the best-response problem of a player and construct an iterative algorithm to solve the game. Empirical analysis shows exponential convergence towards the Nash equilibrium. A comparison to a DSM scheme with a static game, reveals the advantages of the dynamic game approach. We provide an extensive analysis on the influence of the forecasting error on the outcome of the game. A key result demonstrates that our approach is robust even in the worst-case scenario. This grants considerable gains for the utility company organising the DSM scheme and its participants.

==> sec/4_results.tex <==
%results
In this section, we firstly summarise important simulation parameters and introduce the specific data sets for electricity demand and generation from the photovoltaic (PV) installation. Secondly, all results are shown with detailed explanations of the individual parameters under investigation. Thirdly, the results are discussed and compared to the literature.
The correctness of the implementation of Algorithm~\ref{alg:bestResponse} is provided in the Appendix~\ref{sec:convResults}.


\subsection{The Simulation Setup}
\label{sec:simSetup}
In the real-world application, the smart meter of individual households collects data about electricity demand and generation from the available PV installation. As specified in Section~\ref{sec:smartGrid}, the demand-side management (DSM) protocol requires participants to send forecasts of the demand and generation to the utility company. These forecasts are based on historically collected data. In order to run our simulations, we omit this forecasting step and rather make use of two publicly available data sets.

\paragraph{Demand data:}
The demand data stem from the openei dataset~\cite{Openei2013a}. It contains 365 days of simulated hourly data\footnote{We make use of $T=24$ for all simulations, if not stated otherwise.} for households in TMY3-locations in the USA~\cite{Nrel2015}. The building models used for this simulation can be found in~\cite{Openei2013}. Based on an additional survey, all buildings are put into one of three different category. They differ with respect to their overall consumption. Following~\cite{Openei2013a}, we refer to them as LOW, BASE and HIGH consumers. For all simulation runs, we picked the same $M=25$ households, in close vicinity to each other, to represent our neighbourhood. With respect to their consumption categories, we have seven LOW, nine BASE and nine HIGH users. 

\paragraph{PV data:}
Data for the PV generation are based on real-world measurements~\cite{PowerNetworks2014} in the UK. They contain hourly values for days between September 2013 and October 2014. Note that latitude and climate zone of the measurement location are similar to the ones of the demand data. In assumption that the weather for all households in the neighbourhood is the same, we use data from the same site for each of them. An estimate for the $kW\!p$ value is obtained from looking at the highest hourly output in the course of a whole year. Its value is $w_{\max}=3.7\;$kWh, which is why we assume $kW\!p\approx 4\;$kW. We account for different sizes of PV installations by scaling the data set with a household specific factor $p_{n}$. About $6\%$ of the collected data was corrupted. We set all these values to $w=0.0\;$kWh. This does not pose any problem for our simulation results, but can be seen as realistic failures of the installation. 

\paragraph{Battery and pricing parameters:} The parameters of the battery are based on the Tesla Powerwall 2~\cite{Tesla2017} data sheet. The choice to employ this battery system is motivated by two reasons: (i) The same battery was used in~\cite{Pilz2017}, allowing for a direct comparison of the results. (ii) A non-extensive analysis of different battery systems showed that the Tesla Powerwall 2 qualifies as a representative of state-of-the-art technology. Please see the Appendix~\ref{sec:batteryJust} for more details. A summary of the battery parameters can be found in Table~\ref{tab:batPara}. The data sheet only specifies the round-trip efficiency $\eta = \eta^+\cdot\eta^-$ of the battery. Without loss of generality, we assume that charging and discharging contribute equally, yielding $\eta^+ = \eta^- = \sqrt{0.918}$. 

\begin{table}[t]
	\caption{\textit{Battery parameters.} Parameters for a Tesla-inspired~\cite{Tesla2017} home battery storage system.}
	\centering
	\label{tab:batPara}
	\begin{tabular}{cc}
		\toprule
		\textbf{Variable}	& \textbf{Value}	\\
		\midrule
    	$\eta^+$ & $0.958$\\ 	
    	$\eta^-$ & $0.958$\\
    	$\eta_{\text{inv}}$ & $0.960$\\
		$\rho^+$ & $5.0$\;kW/h\\   
    	$\rho^-$ & $-7.0\;$kW/h\\
		$\bar{\rho}$ & $-0.001$\\
    	$s_{\max}$ & $13.5$\;kWh \\
    	$s_{\min}$ & $0.0$\;kWh\\
    	$s^*$ & $9.46$\;kWh\\
		\bottomrule
	\end{tabular}
\end{table}
For the parameters in the cost function~\eqref{eqn:costFunction} we use $c_2 = 0.03125\;$\$/MW$^2$, $c_1=1.0\;$\$/MW, and $c_0=0$, following other studies~\cite{Pilz2017,Rahbar2015}. This allows to compare our results. %Households that do not participate in the DSM scheme pay $p=\todo{100}\;$\$/MW.


\subsection{Results}
\label{sec:results}
We compare the game--theoretic approach introduced in this manuscript (cf.~Section~\ref{sec:game}) with a simpler non-cooperative static game, revealing the advantages of the dynamic treatment. Subsequently, the analysis of how the participation rate of the DSM scheme and the forecasting errors influence the scheduling outcome is shown. Finally, we consider the influence of the composition of the neighbourhood on the peak-to-average ratio (PAR) reduction.
This is an important measurement of the effectiveness of the DSM scheme. We consider the PAR of the aggregated electricity load \eqref{eqn:totalLoad} over the respective scheduling period. It is defined by
\begin{equation}
	\text{PAR} = T\cdot\frac{\max_{t\in\mathcal{T}}L^t}{\sum_{t\in\mathcal{T}}L^t}\ .
	\label{eqn:PAR}
\end{equation}


\subsubsection{Comparison Between a Static and a Dynamic DSM scheme}
\label{sec:resultsComparison}
In~\cite{Pilz2017}, a similar DSM scheme to the one described in Section~\ref{sec:smartGrid} was examined. 
Both are based on a battery scheduling game for households of a neighbourhood served by the same utility company (UC). Their main difference is the underlying game that determines the schedules for the upcoming day. Whereas in this paper we employ a discrete time dynamic game,~\cite{Pilz2017} made use of a simpler non-cooperative static game in which players were only able to choose between four discrete options for each interval. For a more thorough description please see~\cite{Pilz2017}. For the sake of comparison, none of the households is equipped with PV cells.
\begin{figure}[t]
	\centering 
	\subfigure[week 12\label{fig:week12load}]{\includegraphics[trim=0 0 0 0,clip,width=0.81\linewidth]{./fig/week12_comparison.pdf}}
	\subfigure[week 38\label{fig:week38load}]{\includegraphics[trim=0 0 0 0,clip,width=0.81\linewidth]{./fig/week38_comparison.pdf}}
	\vspace{-0.5\baselineskip}
	\caption{\textit{Load comparison.} The aggregated load of all households in the neighbourhood is plotted over time. The simulation domains cover seven days, that were each scheduled consecutively. The aggregated demand is given as a reference. The orange curve results from a DSM scheme employing a static scheduling game~\cite{Pilz2017}, while the green one stems from a DSM scheme employing a dynamic game. Other than the underlying game structure, all parameters are identical.}
	\label{fig:LoadComparison}
\end{figure}
\begin{table}
\caption{\textit{PAR comparison.} Peak-to-average ratios calculated as the average over the individual days of week~12, week~25, week~38, and week~51 for the case without storage system (Reference) and both underlying games of the DSM scheme. $\mu$ gives the average over all four weeks. Static: game employed in~\cite{Pilz2017}; Dynamic: game described in Section~\ref{sec:game}. The values in parentheses represent the standard deviation.}
	\label{tab:comparePAR}
	\centering
	\begin{tabular}{ccC{2.3cm}C{2.3cm}C{2.3cm}}
		\toprule
		&	& \textbf{Reference} & \textbf{Static} & \textbf{Dynamic} \\
		\midrule
    	\multirow{4}{*}{\textbf{Period}} & week 12 & $1.623$ $(0.005)$ & $1.374$ $(0.070)$ & $1.013$ $(<\!0.001)$ \\
    	&week 25 & $1.574$ $(0.033)$ & $1.410$ $(0.035)$ & $1.198$ $(0.016)$ \\
    	&week 38 & $1.685$ $(0.031)$ & $1.439$ $(0.080)$ & $1.231$ $(0.015)$ \\
    	&week 51 & $1.718$ $(0.037)$ & $1.468$ $(0.082)$& $1.015$ $(0.001)$ \\ \midrule
    	&$\mu$ & $1.650$ $(0.064)$ & $1.423$ $(0.040)$ & $1.114$ $(0.117)$\\
	\bottomrule
	\end{tabular}
\end{table}

In this subsection, we compare the two approaches with respect to their success in reducing the PAR of the aggregated load. To this end, the same parameters for each household and also the same demand data are used. Households do not have the capability of on-site generation, but are equipped with the same batteries (cf.~Table~\ref{tab:batPara}). The upcoming day is divided into $T=12$ intervals and we assume $N=M=25$, i.e.~every household takes part in the DSM scheme. As in~\cite{Pilz2017}, we simulate full weeks by using the state-of-charge (SOC) values of the batteries at the end of the scheduling period as the initial configuration for the following one. Figure~\ref{fig:week12load} and Figure~\ref{fig:week38load} show the aggregated load curves achieved by the DSM schemes for forecasts given by week 12 and week 38 of the demand data set~\cite{Openei2013a}, respectively.
For completion, we also simulated week~25 and week~51 as done in~\cite{Pilz2017}. A summary of the achieved results can be seen in Table~\ref{tab:comparePAR}.
\begin{figure}[t]
	\centering 
	\subfigure[static scheduling game\label{fig:comp_discrete}]{\includegraphics[trim=0 0  0 0,clip,width=0.45\linewidth]{./fig/NEW_discrete_small.pdf}}
	\subfigure[dynamic scheduling game\label{fig:comp_dynamic}]{\includegraphics[trim=0 0 0 0,clip,width=0.45\linewidth]{./fig/NEW_dynamic_small.pdf}}
	\vspace{-0.5\baselineskip}
	\caption{\textit{Nash equilibrium schedule comparison.} The schedules for all participating households of the demand-side management scheme for a single scheduling period (week 38, day 5, cf.~\cite{Pilz2017}) are shown together with their respective aggregated load and aggregated state-of-charge (SOC). (a) The underlying game structure is a static non-cooperative game from~\cite{Pilz2017}. Within each interval, players can choose between four discrete decisions. (b) Here, the game structure is the dynamic game introduced in Section~\ref{sec:game}. Note that the schedules employ the same scaling.}
	\label{fig:comparison}
\end{figure}

On average, a $14\%$ and a $32\%$ decrease of the PAR value was achieved by the static and the dynamic games, respectively. To understand the differences of the outcomes, we explicitly look at the schedules that are obtained in the NE of the respective games. Figure~\ref{fig:comparison} shows these schedules exemplarily for day 5 of week 38 (Figure~\ref{fig:week38load}, cf.~Figure 3 in~\cite{Pilz2017}) together with the aggregated load and aggregated SOC above it. Each row illustrates the equilibrium schedule of one household. 


\subsubsection{Influence of Participation Rate and Forecasting Errors}
\label{sec:parRate_Error}
The question of how many participants are needed to obtain considerable gains in terms of PAR reduction and savings is important. 
\begin{figure}[th]
	\centering
  	\includegraphics[width=0.79\textwidth]{./fig/PARvsNM_barNEW.pdf}
  	\caption{\textit{Peak-to-average ratio (PAR) reduction dependency on the participation rate.} The mean PAR reduction in per cent is plotted over the participation rate in per cent. The right-hand axis shows the absolute values of the PAR. In addition to the average over 365 days, the standard deviation is shown for each data point. The simulations were run for a scenario with forecasting errors and one without forecasting errors. Note that the data points are slightly shifted along the abscissa to increase readability.}
  	\label{fig:PARvsNM}
\end{figure}
\begin{figure}
	\centering
  	\includegraphics[width=0.79\textwidth]{./fig/savingVSnm.pdf}
  	\caption{\textit{Savings dependency on the participation rate.} The mean bill reduction in per cent for participants of the demand-side management scheme are plotted over the participation rate in per cent. In addition to the average over 365 days and participants, the standard deviation between different participants is shown for each data point. The simulations were run for a scenario with forecasting errors and one without forecasting errors. The difference between the two curves is plotted against the right-hand axis.}
  	\label{fig:savingVsNM}
\end{figure}
Moreover, within this subsection the robustness with respect to the forecasting errors (cf.~Section~\ref{sec:error}) is shown. To do so, we assume the forecasting error for the demand to be $\epsilon_d = 8\%$ for every household~\cite{Bichpuriya2016}\reviewAdd{, which could be obtained from a forecast performed by an artificial neural network, and is approximately 2.5 times higher than the best forecast obtained by them}. This is independent of whether the household participates in the DSM scheme or not. The forecasting error for the solar generation is set to $\epsilon_w = 10\%$ in accordance with~\cite{Dolara2015,Rana2016}. \reviewAdd{Rana\etal~\cite{Rana2016} make use of a neural network and clustering of weather data to forecast half hourly solar power output for the upcoming day.} Note that only participants of the DSM scheme are equipped with PV cells and thus subject to the forecasting error. The values are taken to represent a worst-case scenario. Subsequently, any real-world scheduling result should fall in the interval between the worst-case outcome and the respective outcome without any forecasting error.

%\paragraph{PAR reduction:} 
We simulate a full year and average over the obtained PAR values for the individual days. All participants are equipped with a lithium-ion battery (cf.~Table~\ref{tab:batPara}) and a solar cell. The size of the PV installation depends on the user's category. For LOW, BASE, and HIGH consumers, we use $p_n=0.3$, $p_n=0.5$, and $p_n=0.7$, respectively. Starting with all 25 households taking part in the DSM scheme, we eliminated three users, i.e.~one randomly selected from each consumer category, in each subsequent run. Non-participant still exhibit the specified forecasting error for their demand. 


Figure~\ref{fig:PARvsNM} shows the reduction of the PAR value over the rate of participating consumers for the scenarios with and without forecasting errors. It includes not only the mean values, but also the standard deviation. Note that we slightly shifted the results for both runs along the abscissa to increase readability. An additional axis on the left indicates the absolute PAR values.
%\paragraph{Savings:} 
Whereas the PAR reduction is the interest of the UC, the financial rewards, i.e.~savings off the energy bill, are the interests of the participants of the DSM scheme. Figure~\ref{fig:savingVsNM} shows the average saving per day for all participants both with and without forecasting error. For further insight, it also illustrates the difference between the two curves. 



\subsubsection{Consumer Type Dependency}
\label{sec:resultsConsumer}
\begin{figure}[thb]
	\centering
  	\includegraphics[width=0.79\textwidth]{./fig/PARvsNM_compare.pdf}
  	\caption{\textit{Peak-to-average ratio (PAR) reduction for different neighbourhoods.} The mean PAR reduction in per cent is plotted over the participation rate in per cent for different mono-type consumer neighbourhoods. In addition to the average over 365 days, the standard deviation is shown for each data point. For comparison, the results of a mixed neighbourhood (cf.~Figure~\ref{fig:PARvsNM}) are also presented. Note that the data points are slightly shifted along the abscissa to increase readability.}
  	\label{fig:comparison_PARcons}
\end{figure}
\begin{figure}[thb]
	\centering
  	\includegraphics[width=0.79\textwidth]{./fig/bill_comp.pdf}
  	\caption{\textit{Savings for different neighbourhoods.} The mean bill reduction in per cent for participants of the demand-side management scheme are plotted over the participation rate in per cent for different mono-type consumer neighbourhoods. In addition to the average over 365 days and participants, the standard deviation between different participants is shown for each data point. For comparison, the results of a mixed neighbourhood (cf.~Figure~\ref{fig:savingVsNM}) are also presented.}
  	\label{fig:comparison_bill}
\end{figure}
The results in Section~\ref{sec:resultsComparison} and Section~\ref{sec:parRate_Error} are all based on a neighbourhood consisting of a mix of the three different consumer types (LOW, BASE, HIGH). Figure~\ref{fig:comparison_PARcons} shows the possible PAR reductions for mono-type neighbourhoods. To allow for comparison $M=25$ is kept constant. Furthermore, we use the same forecasting errors of $\epsilon_d=8\%$ and $\epsilon_w=10\%$ for the demand and renewable energy generation, respectively (cf.~Section~\ref{sec:parRate_Error}). All the simulations consider a scheduling period of a full year. 

We also calculated the average savings that are achieved by the participants of the DSM scheme. These results are presented in Figure~\ref{fig:comparison_bill} together with the reference of a mixed neighbourhood (cf.~Figure~\ref{fig:savingVsNM}) with forecasting errors.


\newpage
\subsection{Discussion}
\label{sec:discussion}
For each subsection of the results (cf.~Section~\ref{sec:results}), there is a corresponding subsection discussing these outcomes.


\subsubsection{Comparison Between a Static and a Dynamic DSM scheme}
\label{sec:discCompare}
Comparing the aggregated load curves (cf.~Figure~\ref{fig:LoadComparison}) shows that a DSM scheme based on a dynamic game can achieve an almost flat profile. Nevertheless, depending on the given data, the outcome of the scheduling is subject to a finite-horizon effect. Empirically, we observe peaks and troughs at the end of the scheduling period if the demand for the final interval is lower than the average demand of the whole day. This indicates that the starting time of the DSM scheme has an influence on the achievable outcome. Nonetheless, this parameter is fixed through the DSM scheme protocol, thus asking for alternative solutions to the finite-horizon effect. Future work will aim to eliminate the influence of the starting time altogether.

In Table~\ref{tab:comparePAR}, we observe that on average the dynamic game reduces the PAR value more than twice as much as the static game. However, with respect to the individual weeks the static game shows a smaller standard deviation of 0.04 and thus seems to be more consistent. Its achieved reductions are all between $10.4\%$ -- $15.3\%$, while the range of reductions by the DMS scheme with the dynamic game is $23.9\%$ -- $40.9\%$. The differences with respect to the standard deviations is again owed to the finite-horizon effect. It is also present in the case with the static game, but due to generally worse outcome, does not alter it as much as the results of the dynamic scheduling game.

We can further understand the differences between the static and dynamic game from Figure~\ref{fig:comparison}. The restriction to four discrete options for each interval in the static case, i.e.~(i) remain idle, (ii) charge half interval, (iii) charge full interval, and (iv) use battery, results in a majority of intervals where the battery remains idle. This is because of a lack of incentive to charge the battery by the two given amounts. In the dynamic game, players can choose to charge their battery from a continuous spectrum of decisions in a given interval. This difference becomes most apparent when looking at the aggregated SOC of all participants. Whereas the maximal SOC in the static case is approximately $64\;$kWh, almost twice as much ($120\;$kWh) is charged in the dynamic case. In summary, it shows that the increased flexibility of the dynamic game is better suited to minimise the PAR of the aggregated load.

\reviewAdd{Note that all these comparisons allow for strong conclusions as they are based on the identical data set~\cite{Openei2013a} and also all the other parameters, such as number of players $N$, number of time intervals $T$, etc. are chosen to be the same. Nevertheless, comparisons to other results in the literature are possible: Compared to the work by Nguyen\etal~\cite{Nguyen2015}, a better PAR reduction is achieved while also the number of iterations to obtain the equilibrium solution is lower by two orders of magnitude. Similarly, the PAR reduction of Yaagoubi\etal~\cite{Yaagoubi2015b} is worse than the approach shown in this manuscript. As they schedule not only the battery but also shift other household appliances, a comparison of the computational costs is not appropriate.}


\subsubsection{Influence of Participation Rate and Forecasting Errors}
\label{sec:discPARvsNM}
Although a worst-case scenario is simulated, the outcome with respect to PAR reduction (cf.~Figure~\ref{fig:PARvsNM}) and electricity bill (cf.~Figure~\ref{fig:savingVsNM}) reduction show considerable gains for the UC and the participants of the DSM scheme. \\

%\paragraph{PAR reduction:} 
Without forecasting error the PAR reduction monotonically improves with the proportion of the participants. This stands in contrast to the results shown in~\cite{Soliman2014}, where a minimum is reached at medium range participation rate. In comparison to other studies, such as~\cite{Nguyen2015,Longe2017}, we conclude that our dynamic game performs as good as their respective scheduling approach. At 100$\%$ participation rate, a reduction of $-33.3\%\ (5.8\%)$ is achieved, in agreement with the results shown in Section~\ref{sec:resultsComparison}. It should be noted that a perfectly flat load profile corresponds to an approximately $-40\%$ reduction of the PAR. Thus the outcome is close to the theoretical optimum. When looking at the standard deviation, we observe that it is lowest for the simulation run with 52$\%$ participation rate and increases towards both ends of the spectrum. On the lower end of participation rate the fluctuations of the PAR value for different days is just an artefact of the data set in use. Small numbers of participants have not enough influence on the overall neighbourhood to change this. When regarding large participation rates, the PAR value is considerably reduced. The increase of the standard variation for these runs stem directly from the finite-horizon effect already discussed in Section~\ref{sec:discCompare}. 

\begin{figure}[thb]
	\centering
  	\includegraphics[width=0.79\textwidth]{./fig/PARvsError.pdf}
  	\reviewAdd{\caption{\textit{Influence of forecasting error on the achieved PAR value.} The PAR values for three different participation rates are plotted over the forecasting error. Here the abscissa refers to the worst-case scenario as described in Section~\ref{sec:parRate_Error}, e.g. at 0.6 a forecasting error with the magnitude of 60$\%$ of the worst-case is assumed. In the reference case no game is played, so the forecasting error does not influence the PAR value.}}
  	\label{fig:PARvsError}
\end{figure}

The results for runs with forecasting errors follow the results without errors closely. \reviewAdd{Figure~\ref{fig:PARvsError} shows how the forecasting error affects the achieved PAR values for three selected participation rates when transitioning from the perfect forecast to the worst-case scenario as depicted in Figure~\ref{fig:PARvsNM}.} For low participation rates the difference is negligible but starts to increase when more households participate in the DSM scheme. Nevertheless, even in the worst-case scenario, a reduction of $-27.8\%\ (8.9\%)$ is achieved at 100$\%$ participation rate \reviewAdd{(cf.~Figure~\ref{fig:PARvsNM})}. With respect to the standard deviation, we again recognise similarities to the runs without forecasting errors. Smallest variations in the PAR reduction are obtained for participation rates around $50\%$, while we again see increasing variations at high participation rates. Here, the increase is distinctly larger than in the other runs. The reason behind this difference is directly explained by the forecasting error. As more participants join the DSM scheme, the absolute amount of deviation from the actual demand and production is increasing. 

It is worth noting that the result for a participation rate of $76\%$, i.e. a reduction of $-27.7\%\ (4.4\%)$ \reviewAdd{(cf.~Figure~\ref{fig:PARvsNM})}, are very promising from a practical point of view. The UC might not be able to convince everybody to participate in the DSM scheme, but can still gain reductions of the PAR value close to what is achievable at maximum participation.

\reviewAdd{In~\cite{Pilz2018a} it is investigate what happens when no forecast is calculated. Instead the demand data of the current day is used as the input to the dynamic game that determines the schedules for the next day. It turns out that this approach is oversimplified and results in distinctly worse outcomes (cf.~\cite[Figure 5]{Pilz2018a}), i.e.~it shows the importance of a suitable forecasting mechanism.}\\

%\paragraph{Savings:} 
The savings that participants of the DSM scheme can gain increase monotonically with the share of participants. Furthermore, we observe that the variations between different participants is negligible. This is due to the particular proportional billing scheme employed in the scheme (cf.~Section~\ref{sec:utility}). It ensures fairness in the sense that LOW and HIGH consumers can gain equally by signing up for the DSM scheme. The difference between runs with and without forecasting errors reveals that the forecasting error does not influence the bill reduction to a great extent. Since the two curves are almost non-separable to the unaided eye, the difference is shown in the same plot (cf.~Figure~\ref{fig:savingVsNM}). It becomes clear that the difference is actually decreasing for larger numbers of participants. 

This highlights that the dynamic scheduling game ensures robust and beneficial results for the participants of the DSM scheme, even in the worst-case scenario.


\subsubsection{Consumer Type Dependency}
\label{sec:discConsumer}
\begin{figure}[thb]
	\centering
  	\includegraphics[width=0.69\textwidth]{./fig/PARvsNM_compareDiff.pdf}
  	\caption{\textit{Differences between neighbourhoods in peak-to-average ratio (PAR) reduction.} The values shown are based on the results represented in Figure~\ref{fig:comparison_PARcons}.}
  	\label{fig:discComparison_PARcons}
\end{figure}
When comparing different compositions of neighbourhoods, we can gain further insight into the conditions for which the DSM scheme works most efficiently. At first glance, Figure~\ref{fig:comparison_PARcons} reveals that given a low rate of participants in the scheme, the actual type of consumer is not crucial. Figure~\ref{fig:discComparison_PARcons} shows the difference between the respective results for mono-type neighbourhoods and a mixed neighbourhood. A closer look shows that mono-LOW communities are always worse in reducing the PAR value of the aggregated load than any of the other ones. The results in terms of both the mean PAR reduction and the standard deviation get even worse with more than two thirds of households participating in the scheme. Similar observations for mono-type neighbourhoods are found in~\cite{Soliman2014}.

For both mono-BASE and mono-HIGH neighbourhoods it can be observed that they perform better ($<1$\%) in an interval of medium participation rate than the mixed neighbourhood. Nevertheless, at $N=M$ the obtained PAR reduction is smaller by 1.8$\%$ and 4.5$\%$, respectively. Considering the variation of these mean PAR reduction values, it becomes clear that it is most beneficial to have a mixed-consumer neighbourhood.\\

Figure~\ref{fig:comparison_bill} shows the average bill reduction for the participants of the DSM scheme for different participation rates. Generally, they show the same behaviour already observed in Figure~\ref{fig:savingVsNM}. The influence of the proportionality factor in the billing scheme \eqref{eqn:billDSM} is clearly visible. Although the mixed-consumer neighbourhood achieves better PAR reduction, the average savings are almost identical to a mono-BASE neighbourhood. A neighbourhood that purely consists of HIGH consumers can save about 11$\%$ off the energy bill and is consistently most rewarding for the participants independent of the participation rate.























